Provable and Efficient Continual Representation Learning

In continual learning (CL), the goal is to design models that can learn a sequence of tasks without catastrophic forgetting. While there is a rich set of techniques for CL, relatively little understanding exists on how representations built by previous tasks benefit new tasks that are added to the network. To address this, we study the problem of continual representation learning (CRL) where we learn an evolving representation as new tasks arrive. Focusing on zero-forgetting methods where tasks are embedded in subnetworks (e.g., PackNet), we first provide experiments demonstrating CRL can significantly boost sample efficiency when learning new tasks. To explain this, we establish theoretical guarantees for CRL by providing sample complexity and generalization error bounds for new tasks by formalizing the statistical benefits of previously-learned representations. Our analysis and experiments also highlight the importance of the order in which we learn the tasks. Specifically, we show that CL benefits if the initial tasks have large sample size and high "representation diversity". Diversity ensures that adding new tasks incurs small representation mismatch and can be learned with few samples while training only few additional nonzero weights. Finally, we ask whether one can ensure each task subnetwork to be efficient during inference time while retaining the benefits of representation learning. To this end, we propose an inference-efficient variation of PackNet called Efficient Sparse PackNet (ESPN) which employs joint channel & weight pruning. ESPN embeds tasks in channel-sparse subnets requiring up to 80% less FLOPs to compute while approximately retaining accuracy and is very competitive with a variety of baselines. In summary, this work takes a step towards data and compute-efficient CL with a representation learning perspective. GitHub page: https://github.com/ucr-optml/CtRL

==> sec/algo.tex <==
\begin{algorithm}[t]\caption{Efficient Sparse PackNet (ESPN)}
    \begin{algorithmic}[1]
    \Require{}
    Task sequence $\{\Tc_t\}$; constraints $\OFLOP_t,\ONNZ_t$; step size $\eta$; pre-training, pruning, fine-tuning durations.
    
    \State List of task masks $\Mc\gets\emptyset$.
    %\State Set initial $\m$ equal to all True's; initial percentage of nonzeros in scaler factor $p=1$.
    \State \texttt{\comc{\% Initially all weights are free}}%\textcolor{black}
    \State Set of free weights {$\mf\gets[p]$}
    %\State Set initial $\M$ equal to all \texttt{True}'s. 
    \For {$\Tc_t \in \{\Tc_t\}$}
    \State \texttt{\comc{\% Pretrain over all free weights}}
    \While {pre\_training}
    \State $\bt\leftarrow\bt-\eta\cdot\nabla\Lc_{\Sc_t}(\bt)\odot \mf$
    \EndWhile
    \State Determine the sequence of FLOP, nonzero (NNZ) 
    \State targets for pruning iterations: $\OFLOP_t^{\text{iter}}, \ONNZ_t^{\text{iter}}$
    \State \texttt{\comc{\% Weight \& channel pruning for $\m_t$}}
    %\State \texttt{\comc{\% Each iteration prunes $\m_t$}}
    \For {{iter \textbf{in} pruning\_iter}}
    \State Channel pruning: $\FLOP(\m_t)\leq\OFLOP_t^{\text{iter}}$
    \State Weight pruning:~~~{$\NNZ(\mnt)\leq\ONNZ_t^{\text{iter}}$}
    \State $\bt\leftarrow\bt-\eta\cdot\nabla\Lc_{\Sc_t}(\bt)\odot (\mf\cap\m_t)$
    \EndFor
    %\State $\hat\m_t\leftarrow\m_t$
    \State \texttt{\comc{\% Fine-tune the free weights in $\m_t$}}
    \While {fine\_tuning}
    \State $\bt\leftarrow\bt-\eta\cdot\nabla\Lc_{\Sc_t}(\bt)\odot(\m_t\cap\mf)$
    \EndWhile
    \State \texttt{\comc{\% Save the mask of $\Tc_t$}}
    \State $\Mc\leftarrow\Mc\cup\{t:\m_t\}$
    \State \texttt{\comc{\% Remove the weights in $\m_t$}}
    \State $\mf\leftarrow\mf \setminus \m_t$ % \Comment here consider $\Mc^{(\tau)}$ as binary mask
    % \State Update $\M$ depending on $\Mc^{(\tau)}$ \Comment zero entries are free channels in $\Mc's$
    %\State Freeze the weights of the masked channels.
    \EndFor
    %\State Each task $\mathcal T_\tau$ has a ($\Mc^{(\tau)}, \Gamma^{(\tau)}$) pair for inference and each inference is under FLOPs restriction.
    \end{algorithmic}\label{algo 1}
\end{algorithm}
\ylm{why we use $\mf$ here. It is confused with model function}
\ylm{Should we add additional intro that we prune $\m_t$ to achieve targets?}

==> sec/exps.tex <==
\section{Experimental Evidences in CL}\label{sec:exp}

%In Table~\ref{CIFARtable}, we present results for two individual-trained models with different FLOPs level: individual-1 trains each task over original model without any channel or weights pruning, while individual-0.2 trains 20 models for 20 tasks individually and conduct gradual channel pruning as Algo. \ref{algo 1} to meet $20\%$ FLOP constraint. 


%\Salnote{Do not understand the last line.}

%Part A: 




%\input{sec/fig_mnist}
% where 20 tasks have separate \red{classification heads}
%\Salnote{This terminology of FLOPs restricted to 20\% seems strange to me.}
%(shown in red dotted) or without (shown in green dotted) FLOPs restriction
% with 20\% of computation and performance is almost preserved. 

%which is not as reflective of real world \cite{farquhar2018towards}
%can generate hundreds of tasks by different random permutation matrix. However 


%\input{sec/fig_rep}
% We evaluate our algorithm on three different datasets. In the first experiment, following the same setting in \cite{}, we use SplitCIFAR100-20 tasks. We randomly split original CIFAR100 dataset into 20 tasks, each with 5 classes, 2,500 training samples and 500 test samples. 




\subsection{Investigation of Data Efficiency}%\noindent\textbf
To investigate how features learned from earlier tasks help in training new tasks in continual representation learning, we introduce a new experimental setting based on SplitCIFAR100 described in Sec~\ref{sec:setting} where 100 classes are randomly partitioned into 20 5-class classification tasks. Let us denote the original $20$ tasks as $\Tc_1,...,\Tc_{20}$. First, we split the tasks into a continual learning task set $\Dc_{cl}=\{\Tc_1,..,\Tc_{15}\}$ and a test task set $\Dc_t=\{\Tc_{16},...,\Tc_{20}\}$. Tasks in $\Dc_{cl}$ {retain} all $2500$ training samples per task. To test the data efficiency of CL, $\Dc_t$ tasks only have 10\% of their original training samples (i.e., $250$ for each task). We use ResNet18 described in Sec~\ref{sec:setting}. To quantify the benefits of learned feature representations in the continual learning process, we train the network sequentially using tasks in $\Dc_{cl}$ and test knowledge transferability separately over $\Dc_t$ after each task in $\Dc_{cl}$ added to the network. \red{Our goal is to quantify the benefits of learned feature representations in the continual learning process. To this aim, we train the network using samples from test tasks in $\Dc_t$ after every task in $\Dc_{cl}$ and use the test accuracy of $\Dc_t$ as a proxy for quantifying the quality of representations learned in previous tasks}.
%
\input{sec/fig/cifar_oc}


First, we use the CL method to sequentially learn tasks $\Dc_{cl}$ and save the supernet after every task. In this manner, we get 16 different supernets $\s_0,\s_1,...,\s_{15}$, where $\s_0$ stands for the initial supernet with no task, and $\s_i$ stands for the supernet after training $\Tc_1,\dots,\Tc_i$ using CL algorithm for $i\leq 15$. The source of the knowledge in $\s_i$ is the first $i$ tasks of the $\Dc_{cl}$ dataset. The test dataset $\Dc_t$ is used to test the transferability of the knowledge contained in supernet $\s_i$. {We separately train each of the 5 tasks of $\Dc_t$ by adding them into $\s_i$ in a continual learning manner (i.e.~by preserving the weights trained for $\Dc_{cl}$ \blue{and following the same channel pruning and weight allocation rules}).} This is done for all $16$ supernets $\s_i$. Training at supernet $\s_0$ is equivalent to training the network from scratch. Training at supernet $\s_i$ shows how features learned from $\Tc_1,\dots,\Tc_i$ help the test tasks in terms of data efficiency. We plot the average test accuracy on \blue{$5$ trails in Fig.~\ref{fig:LS} for each $\s_i$ and test accuracy in each trail is averaged over $5$ test tasks.}

%resultsAs shown in Figure~\ref{overview fig}, in this case not all the learned features are reused in new tasks due to the channel selection. Therefore, we run ESPN-1 without FLOPs restriction so that all the trained weights are reused. 
Figure~\ref{fig:LS} summarizes the results of our experiment. Orange and Blue curves display ESPN-1 and ESPN-0.2 results. We also run PackNet, SupSup, and Individual-0.2/-1 baselines using the same setting as in Table~\ref{CIFARtable}\som{ with only difference being weight allocation $\alpha=0.05$ rather than $\alpha=0.1$}. Since SupSup uses a fixed model with random initialization and learns a mask for each task separately, no knowledge is transferred. This is why dashed lines are strictly horizontal. Figure~\ref{fig:LS} shows that ESPN-0.2, ESPN-1, and PackNet methods benefit from features trained by earlier tasks since the test accuracy significantly improves when we train the new task on top of a network containing more continual tasks. Observe that, the performance of ESPN gradually increases with the growing number of continual tasks. This reveals its ability to successfully transfer knowledge from previous learned tasks. \ylm{We believe ESPN's advantage over PackNet arises from the Task-specific BatchNorm weights which allow ESPN to better re-purpose the features learned by earlier tasks. The small gap between ESPN-0.2 and ESPN-1 also shows that our ESPN algorithm performs well in finding the most relevant features despite channel sparsity restrictions.} Complementing these experiments, the next section provides theoretical insights into the representation learning ability of PackNet/ESPN.

%Observe that, ESPN-0.2 may prevent a new task from accessing all previous features (due to FLOPs constraint); thus, perhaps unsurprisingly, ESPN-1 performs slightly better. Results are shown in the orange curve.

\subsection{Importance of task order: diversity and sample size}

\input{sec/fig/sample_size}

==> sec/fig/cifar.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \node at (0,0) [scale=0.8] {\includegraphics[width=\linewidth]{figs/FLOP.pdf}};
        \node at (0,-2.5) [scale=1.0] {\red{FLOPs constraint $\gamma$}};
        \node at (-3.3,0) [scale=1.0,rotate=90] {Accuracy};
    \end{tikzpicture}
	\caption{We display the impact of weight allocation $\alpha$ (Eq.~\eqref{wa-eq}) and FLOPs constraint on task-averaged ESPN accuracy for SplitCIFAR100. Setting $\alpha$ too small (blue curve) degrades performance as tasks do not get enough nonzeros to train on. Setting both $\alpha$ and FLOPs to be large also degrades performance, because the first few tasks gets to occupy the whole supernetwork at the expense of future tasks. %$\alpha=0.1$ strikes a balance between these extremes.
	}
	%does not give enough freedom to tasks decreasing performance. Since FLOPs set the constraint on the model size and $\alpha$ decides the number new trainable weights, setting both of them large leads to a failure where most weights are trained and frozen in first several tasks (green and red lines). On the opposite, the blue line shows that smaller $\alpha$ and FLOPs also lead to a catastrophic failure because there are too few trainable parameters for each task.  	
	
	\label{fig:FLOP}
\end{figure}

==> sec/fig/mnist.tex <==
\begin{figure}[t]
    \begin{subfigure}{1.6in}
        \begin{tikzpicture}
        \node at (0 ,0) [scale=0.23] {\includegraphics{figs/rotated.pdf}};
        \node at (0,-1.75) [scale=0.85] {\# of trained tasks};
        \node at (-2.2, 0) [scale=0.85, rotate=90] {Accuracy};
        \end{tikzpicture}\caption{\small{
        RotatedMNIST
        %Test accuracy when add large number of tasks in RotatedMNIST and experiments. Observe that, the test accuracy remaining high in RotatedMNIST-ESPN displays the ability of continual representation learning in high correlated tasks.
		}}\label{fig:rotated}
    \end{subfigure}\hspace{7pt}\begin{subfigure}{1.6in}
    \centering
        \begin{tikzpicture}
        \node at (0,0) [scale=0.23] {\includegraphics[trim=40 0 0 0, clip]{figs/Permuted.pdf}};
        \node at (0,-1.75) [scale=0.85] {\# of trained tasks};
        \end{tikzpicture}	\caption{\small{
        PermutedMNIST
        % Test accuracy in PermutedMNIST experiments. We remark that test accuracy decrease dramatically since the pixel-level permuted tasks have lower correlation.\\ \\
		}}\label{fig:permuted}
    \end{subfigure} 
    \caption{Results of experiments on RotatedMNIST and PermutedMNIST datasets with FC1024 model. Yellow curves show ESPN-0.2 accuracy and blue curves are PackNet. Both use weight allocation with $\alpha=0.05$. (a) The test accuracy remains high because tasks in RotatedMNIST are highly correlated. (b) The test accuracy decreases over time because the pixel-permuted tasks have lower correlation and the features built for earlier tasks are not useful. % importance of  % \Salnote{Is y-axis on both a,b the same?}
    }\label{fig:mnist}
\end{figure}
\som{Is Figure 3 accuracy of individual task or average acc until that task?}



==> sec/fig/mnist_rebuttal.tex <==
\begin{figure}[h]
\centering
\vspace{-15pt}
\small
    \begin{subfigure}{0.22\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0 ,0) [scale=0.20] {\includegraphics[trim={0 0 2cm 0},clip]{LaTeX/figs/rotated_rebuttal.pdf}};
        \node at (0,-1.5) [scale=1.0] {\# of trained tasks};
        \node at (-1.8, 0) [scale=1.0, rotate=90] {Accuracy};
        \end{tikzpicture}\vspace{-5pt}\caption{{
        RotatedMNIST
        %Test accuracy when add large number of tasks in RotatedMNIST and experiments. Observe that, the test accuracy remaining high in RotatedMNIST-ESPN displays the ability of continual representation learning in high correlated tasks.
		}}\label{fig:rotated}
    \end{subfigure}
    \hspace{-10pt}
    \begin{subfigure}{0.22\textwidth}
        \centering
        \begin{tikzpicture}
        \node at (0,0) [scale=0.20] {\includegraphics[trim={2.3cm 0 2cm 0},clip]{LaTeX/figs/permuted_rebuttal.pdf}};
        \node at (0,-1.5) [scale=1.0] {\# of trained tasks};
        % \node at (-2.2, 0) [scale=1.0, rotate=90] {Accuracy};
        \end{tikzpicture}\vspace{-5pt}\caption{{
        PermutedMNIST
        % Test accuracy in PermutedMNIST experiments. We remark that test accuracy decrease dramatically since the pixel-level permuted tasks have lower correlation.\\ \\
		}}\label{fig:permuted}% \hspace{20pt}
    \end{subfigure} \vspace{-10pt}
    \caption{MNIST experiments.
    }\vspace{-20pt}\label{fig:mnist_rebuttal}
\end{figure}


==> sec/fig/rep.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \node at (0,0) [scale=0.8] {\includegraphics[width=\linewidth]{figs/LS.pdf}};
        \node at (0,-2.5) [scale=1.0] {Supernet};
        \node at (-3.3,0) [scale=1.0,rotate=90] {Accuracy};
    \end{tikzpicture}
	\caption{
	We study the data efficiency in CL using SplitCIFAR100. 15 tasks $\Dc_{cl}=\{\Tc_1,..,\Tc_{15}\}$  with original number of samples are trained with different CL methods to obtain models $s_1$ to $s_{15}$. Here $s_k$ is the supernet after learning first $k$ CL tasks. The remaining 5 tasks $\Dc_t=\{\Tc_{16},...,\Tc_{20}\}$ only have 10\% of their original training samples (250 in total for each task). These are used to test the transferability of the knowledge learned from previous CL tasks starting from model $s_k$ for $0\leq k\leq 15$. We plot the average test accuracy on 5 test tasks. The results show that ESPN and PackNet accuracy greatly benefits from previously learned tasks. Our Theorem \ref{cl thm} provides theoretical intuitions for this observation.
	% ESPN performance gracefully increases for larger $k$. 
	%Observe that, the performance of ESPN gradually increase when increasing the number of learned tasks reveals its outstanding ability on transferring knowledge from previous learned tasks.
	}\label{fig:LS}\vseven
\end{figure}

==> sec/fig/rep_oc.tex <==


\begin{figure}[t]
\vspace{-7pt}
\centering
\begin{minipage}[t]{.38\textwidth}
  \centering
  \begin{tikzpicture}
        \node at (0,0) [scale=1] {\includegraphics[width=\linewidth]{figs/LS.pdf}};
        \node at (0,-2.4) [scale=1.0] {Supernet};
        \node at (-3.1,0) [scale=1.0,rotate=90] {Accuracy};
    \end{tikzpicture}
	\caption{{
	%We study the data efficiency in CL using SplitCIFAR100.
	$15$ SplitCIFAR100 tasks $\Dc_{cl}=\{\Tc_1,..,\Tc_{15}\}$ with original sample sizes are trained with different CL methods to obtain models $s_0$ to $s_{15}$. Here $s_i$ is the supernet after learning first $i$ CL tasks. The remaining 5 tasks $\Dc_t=\{\Tc_{16},...,\Tc_{20}\}$ only have 10\% of their original training samples. These are trained on top of $s_i$ to test the knowledge transfer from previous CL tasks. We plot the average test accuracy on these 5 tasks. The results show that ESPN and PackNet greatly benefits from previously learned tasks. Our Theorem \ref{cl thm} provides theoretical support for these observations.
	% (250 in total for each task)
	%transferability of the knowledge learned
	% for $0\leq k\leq 15$
	% ESPN performance gracefully increases for larger $k$. 
	%Observe that, the performance of ESPN gradually increase when increasing the number of learned tasks reveals its outstanding ability on transferring knowledge from previous learned tasks.
	}}\vspace{-7pt}\label{fig:LS}
\end{minipage}\vseven\vseven
\end{figure}

==> sec/fig/wa.tex <==
% \begin{figure}[t]
% \vspace{-7pt}
% \centering
% \begin{minipage}[t]{.48\textwidth}
%   \centering
%   \begin{tikzpicture}
%         \node at (0,0) [scale=0.8] {\includegraphics[width=\linewidth]{figs/FLOP.pdf}};
%         \node at (0,-2.4) [scale=1.0] {{FLOPs constraint $\gamma$}};
%         \node at (-3.1,0) [scale=1.0,rotate=90] {Accuracy};
%     \end{tikzpicture}
	
% 	%does not give enough freedom to tasks decreasing performance. Since FLOPs set the constraint on the model size and $\alpha$ decides the number new trainable weights, setting both of them large leads to a failure where most weights are trained and frozen in first several tasks (green and red lines). On the opposite, the blue line shows that smaller $\alpha$ and FLOPs also lead to a catastrophic failure because there are too few trainable parameters for each task.  	
	
	
% \end{minipage}%
% \caption{{We display the impact of weight allocation $\alpha$ (Eq.~\eqref{wa-eq}) and FLOPs constraint $\gamma$ on \emph{task-averaged ESPN accuracy} for SplitCIFAR100. Setting $\alpha$ too small (blue curve) degrades performance as tasks do not get enough nonzeros to train on. Setting both $\alpha$ and $\gamma$ to be large also degrades performance (red \& green curves), because the first few tasks get to occupy the whole supernetwork at the expense of future tasks. {Finally $\alpha=0.1$ (orange) achieves competitive performance for all $\gamma$ choices.}} %$\alpha=0.1$ strikes a balance between these extremes.
% 	}\label{fig:FLOP}\vspace{-14pt}
% \end{figure}

==> sec/main_lizzie.tex <==
\subsection{Linear regression}
Consider a linear feature matrix $\vct\Phi=[\vct \phi_1, \vct \phi_2,...,\vct \phi_r]\in\R^{d\times r}$ where $d\gg r$ and $\{\vct\phi_i\}_{i=1}^r$ are orthogonal. Given $\{(\x_{\tau,i},y_{\tau,i})\}_{i=1}^{n_\tau}\sim\Dc_\tau$, describe a linear regression problem as
\begin{align*}
    y=\x^\top\vct\beta+\epsilon~~\text{where}~~\vct\beta=\vct\Phi \w=\sum_{i=1}^r\w_i\vct\phi_i
\end{align*}
where $\w\in\R^r$ and $\epsilon$ is random noise. Therefore we have $\vct\beta\in\text{Span}\{\vct\phi_1,...,\vct\phi_r\}$. Define linear continual regression problem as 
\begin{align*}
    \tau\leq r:&\min_{\vct\phi}\|\X_\tau\vct\phi-Y_\tau\|_2\\
    &\Longrightarrow\hat{\vct\phi}_\tau=(\X_\tau^\top \X_\tau)^{-1}\X_\tau^\top Y_\tau\\
    \tau > r:&\min_{\w}\|\X_\tau\hat\Phi\cdot\w-Y_\tau\|_2~~\text{where}~~\hat{\vct\Phi}=[\hat{\vct\phi}_1,...,\hat{\vct\phi}_r]\\
    &\Longrightarrow\hat{\w}_\tau =((\X_\tau\hat{\vct\Phi})^\top\X_\tau\hat{\vct\Phi})^{-1}\X_\tau\hat{\vct\Phi} Y_\tau
\end{align*}
\subsection{General case}
Consider feature extractor $\phi\in\Phi$ and task-specific function $h\in\Hc$. Denote task predictor $f:=h\circ\phi\in\Hc\times \Phi$, where $\Hc$ and $\Phi$ are continuous search spaces. Let $\phi^M$ be optimal representation that trained from multitasks learning.
\begin{align*}
    \hat\phi^M&=\arg\min_{\phi\in\Phi}\frac{1}{T}\sum_{\tau=1}^T\Lc(h_\tau\circ\phi(\x_\tau),y_\tau)\\
    &\text{s.t.}~~h_\tau=\arg\min_{\h_\tau\in\Hc}\frac{1}{n_\tau}\sum_{i=1}^{n_\tau}\Lc(h_\tau\circ\phi(\x_{\tau,i}),y_{\tau,i})
\end{align*}
In practical problem, $\Phi$ is not uniformly distributed. Here let $\Phi'=(\Phi_1\times\Phi_2\times...\times\Phi_T)$ and assume that for any $\phi\in\Phi$, there exists $\phi'\in\Phi'$ that $\Lc(\phi')-\Lc(\phi)<\eps$.

Define our continual learning problem as
\begin{align*}
    \hat\phi_1&=\arg\min_{\phi\in\Phi_1, h_1\in\Hc}\Lc_{\Dc_1}(h_1\circ\phi)\\
    \hat\phi_\tau&=\arg\min_{\phi\in(\hat\phi_1\times...\times\hat\phi_{\tau-1})\times\Phi_\tau, h_\tau\in\Hc}\Lc_{\Dc_\tau}(h_\tau\circ\phi)
\end{align*}
We will show that for all $\phi\in(\hat\phi_1\times...\times\hat\phi_{\tau-1})\times\Phi_\tau$
\begin{align*}
    Dist(\hat\phi^M,\phi) =\Oc()
\end{align*}
Consider about individual learning that
\begin{align*}
    \hat\phi^I_\tau=\arg\min_{\phi\in\Phi,h_\tau\in\Hc}\Lc(h_\tau\circ\phi)
\end{align*}
Then we will have
\begin{align*}
    Dist(\hat\phi^M,\hat\phi_\tau^I)=\Oc()
\end{align*}



==> sec/prelim.tex <==
\section{Preliminaries}

\textbf{Notation.} Let $\{\Tc_\tau, \tau\in \mathbb N^+\}$ be task identifier and $\Dc_\tau$ be its sample distribution. $\{(\x_{\tau,i},y_{\tau,i})\}_{i=1}^{n_\tau}$ are input-output pairs sampled from $\Dc_\tau$ to generate $\Tc_\tau$ where $n_\tau$ is the sample size.
In the following discussion, we consider $\tau\leq T$ where $T\in\mathbb N^+$.


\subsection{}

\begin{align*}
    \bt^M&:=\arg\min_{\bt}\sum_{\tau=1}^T\sum_{i=1}^{n_\tau}\ell(f(\x_{\tau,i};\bt),y_{\tau,i})\\
    \bt^I_\tau&:=\arg\min_{\bt}\sum_{i=1}^{n_\tau}\ell(f(\x_{\tau,i};\bt),y_{\tau,i})\\
    \bt_\tau^{CL}&:=\arg\min_{\bt,f_\tau}\sum_{i=1}^{n_\tau}\ell(f_\tau(\x_{\tau,i};\bt_{\tau-1}^{CL},\bt),y_{\tau,i})
\end{align*}

==> sec/related.tex <==


\section{Related Work}% \som{Salman helps related work.}

Our contributions are closely related to the representation learning theory as well as continual learning methods. % Due to limited space, the latter discussion is deferred to supplementary.

% \noindent \textbf{Representation learning theory.} The rise of deep learning motivated a growing interest in theoretical principles behind representation learning. Similar in spirit to this project, \cite{maurer2016benefit} provides generalization bounds for representation-based transfer learning in terms of the Rademacher complexities associated with the source and target tasks. {Some of the earliest works towards this goal include \cite{baxter2000model}~and linear settings of \cite{lounici2011oracle,pontil2013excess,wang2016distributed,cavallanti2010linear}.} More recent works \cite{gulluk2021sample,kong2020meta,wu2020understanding,du2020few,tripuraneni2020theory,tripuraneni2020provable,maurer2016benefit,arora2019theoretical} consider variations beyond supervised learning, concrete settings or refine performance bounds. Unlike these existing works, we consider the CL setting and show how the representation learned by earlier tasks help sample complexity of the new tasks. 

\noindent\textbf{Representation learning theory.} The rise of deep learning motivated a growing interest in theoretical principles behind representation learning. Similar in spirit to this project, \cite{maurer2016benefit} provides generalization bounds for representation-based transfer learning in terms of the Rademacher complexities associated with the source and target tasks. Some of the earliest works towards this goal include \cite{baxter2000model}~and linear settings of \cite{lounici2011oracle,pontil2013excess,wang2016distributed,cavallanti2010linear}. More recent works \cite{hanneke2020no,lu2021power,kong2020meta,qin2022non,wu2020understanding,garg2020functional,gulluk2021sample,xu2021statistical,du2020few,tripuraneni2020theory,tripuraneni2020provable,maurer2016benefit,arora2019theoretical,chen2021weighted,sun2021towards} consider variations beyond supervised learning, concrete settings or established more refined upper/lower performance bounds. There is also a long line of works related to model agnostic meta-learning \cite{finn2017model,denevi2019online,balcan2019provable,khodak2019adaptive}. {Unlike these works, we consider the CL setting where tasks arrive sequentially and establish how the representations learned by earlier tasks help learning the new tasks with fewer samples and better accuracy.}

\noindent \textbf{Continual learning.}
A number of methods for continual and lifelong learning have been proposed to tackle the problem of catastrophic forgetting. Existing approaches can be broadly categorized into three groups: replay-based~\cite{lopez2017gradient,borsos2020coresets}, regularization-based~\cite{kirkpatrick2017overcoming, jung2020continual}, and architecture-based methods~\cite{yoon2017lifelong}. \redd{Recent work \cite{ramesh2021model} explores statistical challenges associated with continual learning in terms of the relatedness across tasks through replay-based strategies. In comparison, we focus on the benefits of representation learning and establish how representation built for previous tasks can drastically reduce the sample complexity on new tasks in terms of representation mismatch without access to past data. Another key difference is that our analysis allows for learning multiple sequential tasks rather than a single task.} In our work, consistent with our theory, we focus on zero-forgetting CL~\cite{mallya2018packnet,hung2019compacting,mallya2018piggyback,wortsman2020supermasks,kaushik2021understanding,tu2020extending}, which is a sub-branch of architecture-based methods and completely eliminates forgetting. \cite{hung2019compacting, kaushik2021understanding, mallya2018packnet} train a sub-network for each task and implement zero-forgetting by freezing the trained parameters, while \cite{mallya2018piggyback} trains masks only over pretrained model. Inspired by \cite{ramanujan2020s}, SupSup \cite{wortsman2020supermasks} trains a binary mask for each task while keeping the underlying model fixed at initialization. % that given a enough wide, randomly weighted network, weight mask is the only thing needed to achieve comparable performance. 
%These non-forgetting CL methods have shown very promising results. %and competition 
However in order to embed the super-network with many tasks or to achieve acceptable performance over a masked random network, sufficiently large networks are needed. %For instance, SupSup is among the state-of-the-art methods for CL, but it has to build a binary mask for each new task that has as many entries as the number of parameters in the network. 
Additionally, without accounting for the network structure, the inference-time compute cost of these networks is high even for simple tasks. Our proposed  method is designed to overcome these challenges. In addition to achieving zero-forgetting, our algorithm also provides efficient inference in terms of FLOPs.






%and it also uses specific regularization to update weights. Existing approaches can be broadly categorized into two branches: replay-based \cite{buzzega2021rethinking,aljundi2019gradient,lopez2017gradient,rolnick2018experience,borsos2020coresets}, regularization-based \cite{jung2020continual,kirkpatrick2017overcoming,farajtabar2020orthogonal} and architecture-based methods \cite{yoon2017lifelong,veniat2020efficient}. Replay-based methods focus on efficient sample selection that use minimal amount of samples to represent the original datasets, relularization-based methods work on the regularization algorithm and architecture-based methods are related to neural network selection and model extension. In most cases, more than one branches are used to achieve state-of-the-art results. For example, \cite{lopez2017gradient} use replied samples to calculate gradients of all tasks and update model based on all gradients. \cite{yoon2017lifelong} dynamically expands network upon arrival of new tasks and it also uses specific regularization to update weights. Both replay-based and architecture-extended methods can achieve good results. However, it is only applicable to limited number of tasks or it may run out of memory. What's more, most of current methods try to diminish catastrophic forgetting by updating weights slightly or specifically. 


%Our ESPN algorithm directly targets these shortcomings.
% While we cover the most related works below, see the supplementary material for a more detailed discussion.


==> sec/table.tex <==
\som{Add standard error next to the avg column}
\begin{table*}[h]
    \caption{Continual learning results on SplitCIFAR100 tasks with ResNet18 model using different algorithms. 20 tasks are trained in order. Results for each task is the average accuracy over 5 independent runs. Last column shows the average accuracy for all the tasks with standard error of 5 runs. Individual-0.2/-1 and ESPN-0.2/-0.5/-1 denote the methods with different level of FLOP constraints.}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{
    \begin{tabular}{lcccccccccccccccccccc|c}
    \midrule
    Task ID $\rightarrow$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & avg$\pm$ error\\
    \midrule
    CPG &80.2 &87.9 &92.0 &77.7 &87.7 &81.1 &88.2 &93.8 &87.8 &80.7 &83.3 &86.0 &90.9 &89.4 &81.4 &92.6 &87.2 &90.6 &88.8 &85.5 &86.6$\pm$0.27 \\
    
    RMN &78.5 &83.7 &86.6 &68.4 &85.3 &73.4 &77.8 &88.1 &79.7 &68.3 &71.2 &76.7 &85.2 &79.7 &66.8 &81.8 &70.7 &79.3 &71.9 &72.7 &77.3$\pm$0.07 \\
    
    
 
    % PackNet &78.3 &87.8 &90.7 &76.8 &87.7 &80.7 &88.4 &93.4 &88.9 &83.4 &82.8 &86.9 &92.1 &90.9 &83.3 &93.1 &87.6 &90.2 &89.6 &85.9 &87.9$\pm$0.13 \\
    PackNet &84.5 &89.6 &92.6 &78.7 &89.8 &83.7 &89.2 &94.4 &89.7 &83.5 &84.6 &87.6 &93.0 &91.9 &84.2 &93.2 &86.6 &91.6 &89.7 &86.8 &88.3$\pm$0.10\\
    
    SupSup &86.5 &91.8 &92.9 &81.0 &89.1 &83.4 &88.5 &95.1 &87.8 &83.0 &81.9 &89.0 &94.3 &93.4 &86.6 &94.0 &91.0 &92.6  &91.2 &88.3 &89.1$\pm$0.06\\
    
    \midrule
    % Multitasks & 92.0 &93.8 &96.2 &85.6  &93.2 &87.2  &93.9 &96.8  &91.6 &88.0   &89.8 &92.9 &95.6  &95.6 &88.9 &96.8 &94.6 &96.0 &95.1 &92.9 &92.8 \\
    MTL &89.8 &93.0 &95.2 &82.5 &91.0 &85.7 &92.0 &95.8 &91.3 &86.1 &86.3 &90.0 &94.1 &94.7 &86.7 &95.2 &93.6 &94.8 &92.9 &90.0 &91.0$\pm$0.21\\
    
     % Individual-0.2 &86.2 &89.0 &92.3 &78.9 &87.6 &83.9 &85.5 &93.6 &85.0 &82.7 &81.5 &86.5 &92.8 &91.6 &84.2 &93.8 &89.6 &92.8 &91.2 &88.7 &87.9$\pm$0.10\\
     Individual-0.2 &86.4 &88.8 &93.0 &80.4 &87.5 &85.1 &85.6 &94.7 &85.7 &83.4 &82.3 &88.2 &92.5 &93.2 &85.0 &94.5 &90.5 &92.7 &91.7 &89.5 &88.5$\pm$0.07\\
   
    % Individual-1 &85.2 &88.8 &93.2 &80.0 &87.8 &84.1 &84.8 &93.9 &84.7 &82.0 &81.9 &88.7 &93.1 &92.6 &84.0 &93.0 &90.6 &92.7 &91.4 &88.8 &88.1$\pm$0.12\\
    Individual-1 &86.2 &89.2 &93.2 &79.8 &88.6 &84.1 &85.4 &94.6 &87.0 &82.2 &82.8 &88.3 &93.4 &92.4 &85.6 &94.5 &90.8 &93.0 &92.0 &89.9 &88.6$\pm$0.10\\
    
    \midrule
    % ESPN-0.2 &84.2 &91.3 &93.5 &80.6 &88.2 &83.9 &89.6 &94.8 &89.5 &82.5 &83.4 &87.0 &93.2 &91.6 &83.2 &94.0 &89.4 &91.2 &89.6 &86.4 &\textbf{88.4}$\pm$0.04 \\
    
    ESPN-0.2 &86.4 &90.8 &93.4 &82.4 &89.5 &83.1 &89.8 &95.2 &89.8 &83.5 &85.2 &88.6 &93.7 &92.8 &85.1 &94.8 &88.8 &91.8 &91.2 &86.8 &\textbf{89.1}$\pm$0.12\\
    
    % ESPN-0.5 &84.2 &90.8 &93.7 &80.6 &89.1 &84.4 &90.7 &95.7 &90.3 &84.6 &86.4 &89.0 &93.5 &93.1 &85.3 &95.3 &90.0 &92.3 &91.6 &88.4 &\textbf{89.4}$\pm$0.13 \\
    
    ESPN-0.5 &86.8 &91.3 &94.2 &81.6 &89.2 &84.0 &90.0 &95.7 &90.3 &84.6 &85.3 &89.4 &94.1 &93.0 &85.5 &94.7 &90.2 &93.1 &92.2 &88.8 &\textbf{89.7}$\pm$0.11\\
    
    ESPN-1 &85.0 &91.0 &93.5 &82.3 &89.1 &84.4 &90.2 &95.8 &91.1 &85.2 &86.4 &89.6 &94.3 &93.8 &85.6 &95.4 &90.2 &93.0 &92.9 &88.0 &\textbf{89.8}$\pm$0.14\\
    \midrule
    \end{tabular}}\label{CIFARtable}
\end{table*}

==> sec/table_rebuttal.tex <==
\vspace{-10pt}
\begin{table}[h]
    \caption{Split-TinyImageNet experiments.}\vspace{-7pt}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{
    \begin{tabular}{|c|cccc|}\hline
    method & Individual-0.2 & Individual-1 & ESPN-0.2 & ESPN-1\\\hline
    
    % avg$\pm$error&78.7$\pm$0.08&78.7$\pm$0.11&{79.0}$\pm$0.22&{79.4}$\pm$0.12\\
    
    avg$\pm$error&78.7$\pm$0.08&80.0$\pm$0.18&{79.0}$\pm$0.22&{81.3}$\pm$0.10\\
    
     \hline
    \end{tabular}}\vspace{-10pt}\label{TinyINtable}
\end{table}
